Homophily and Incentive Effects in Use of Algorithms

As algorithmic tools increasingly aid experts in making consequential decisions, the need to understand the precise factors that mediate their influence has grown commensurately. In this paper, we present a crowdsourcing vignette study designed to assess the impacts of two plausible factors on AI-informed decision-making. First, we examine homophily -- do people defer more to models that tend to agree with them? -- by manipulating the agreement during training between participants and the algorithmic tool. Second, we considered incentives -- how do people incorporate a (known) cost structure in the hybrid decision-making setting? -- by varying rewards associated with true positives vs. true negatives. Surprisingly, we found limited influence of either homophily and no evidence of incentive effects, despite participants performing similarly to previous studies. Higher levels of agreement between the participant and the AI tool yielded more confident predictions, but only when outcome feedback was absent. These results highlight the complexity of characterizing human-algorithm interactions, and suggest that findings from social psychology may require re-examination when humans interact with algorithms.

==> sections/results_revised.tex <==

We first analyze the targeting effectiveness of our homophily manipulation. In particular, we asses the impact of this manipulation on participants'
judgements in the first phase of the survey.
We should expect to observe higher agreement between the
participant and the model's predictions on easy cases. 
The mean agreement fractions for
participants' initial and revised binary predictions on these easy cases were both above 80\%.
319 participants (64\%) agreed with the algorithm on all 5 easy cases, and 53 (11\%) agreed for 4-of-5
cases.
%, with higher agreement on high-confidence positive instances (i.e., re-arrests) than on negative ones (92\% vs 73\% for revised predictions). 
However, participants
tended to overpredict the occurrence of re-arrests, 
and agreement on high-confidence positive instances (i.e., re-arrests) was higher than on negative ones (92\% vs. 73\% for revised predictions). 
Similarly to the model's, the predictions made by participants were more accurate for easy cases than difficult ones (classification accuracies were 73\% vs. 45\%). Participants also reported being more certain about their
predictions on the easy cases (3.9 (out of 5) vs. 3.5; p-value of paired t-test$<$0.01). 
In parallel
with agreement, participants' confidence was slightly higher on positive cases compared to negative ones (4.2 vs. 3.6; p-value of paired t-test$<$0.01).
%Unsurprisingly, when the participant observed an AI's recommendation that
%matched their initial binary prediction, confidence in the prediction increased.
Lastly, participants spent longer on difficult cases for both initial predictions (total average time spent on each case was 45s and 40s; p-value of paired t-test$<$0.01). 
 
% I will change this with the actual coefficients estimates
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/agreement_fraction.pdf}
    \includegraphics[width=\linewidth]{figures/switch_fraction.pdf}
  \includegraphics[width=\linewidth]{figures/influence.pdf}
    \caption{Second-phase agreement fraction (top), switch fraction (middle), and mean influence (bottom) for agreement (horizontal axis), incentives (color), and feedback (panels) manipulations (means and 95\% CIs)}
    \label{fig:outcome_metrics_reliance}
\end{figure}

The cleanest tests of our hypotheses are based on responses in the second phase of the experiment: (a) the initial manipulations should have had an impact, and (b) there should not be further learning since participants receive no feedback. 
Figure \ref{fig:outcome_metrics_reliance} shows the agreement fraction, switch fraction, and influence for participants' predictions across treatments in the second phase. 
% to change depending on model
% Since approximately the same number of participants is assigned to each of the interventions, we can assess the impact of homophily via permutation tests controlling for incentives assignments (similarly to Wilcoxon's rank-sum test). 

% We conducted three separate linear regressions---to predict agreement fraction, switch fraction, and influence respectively---with \texttt{homophily}$\times$intervention

% with the medium-high agreement interventions interacted with the presence of asymmetric rewards \texttt{incentives}; all variables also interacted with the presence of outcome feedback. We use robust standard errors for hypothesis testing.  
% The chosen model mirrors our study hypotheses.
% When feedback was absent, the estimates from the three models reveal that low agreement with the model in the initial phase led the lower reliance ([add]).
% Reliance between the remaining homophily interventions (medium and high) was comparable.
% Surprisingly, asymmetric rewards did not substantially increase reliance on the model. 
% When outcome feedback was present, we do not detect any effect of homophily or rewards interventions on agreement.
% Thus, these findings partially align with our hypotheses. 
% In the switch fraction regression, the coefficients
% for  medium homophily manipulation and also its interaction with
% feedback were statistically significant ($\hat{\beta}_{H}^m=0.15$ with $p=0.007$
% and $\hat{\beta}_{HF}^m$=-0.16 with $p=0.005$ respectively). These effects run in
% the expected direction: reliance increased with medium
% levels of homophily but decreased when
% feedback was provided to participants. Surprisingly, we did \emph{not} detect similar effects
% for high homophily ($\hat{\beta}_{H}^h=0.09$ with $p=0.05$ and
% $\hat{\beta}_{HF}^h$=-0.08 with $p=0.136$ respectively). 
% We also found that coefficients for the incentives manipulations were close to 0 and not
% statistically significant. 
% A parallel analysis for influence again yielded analogous results. 
% statistically significant coefficients for medium homophily and its interaction with
% the presence of feedback ($\hat{\beta}_{H}^m=0.11$ with $p=0.022$ and
% $\hat{\beta}_{HF}^m=-0.13$ with $p=0.008$). For influence, the
% coefficient for high homophily was statistically
% significant ($\hat{\beta}_{H}^h=0.11$ with $p=0.023$). 


%We now turn to a brief exploratory analysis of interaction effects between agreement
%and incentives. In Section \ref{sec:experiment}, we hypothesized that an
%asymmetric incentives structure could make participants rely more heavily on the
%AI recommendations when the level of agreement in the initial phase of the survey was high. The patterns in
%Figure \ref{fig:outcome_metrics_reliance} suggest that this may not be the case:
%Participant's reliance does not seem to depend on the exact type of errors on which
%incentives are placed. For example, we observe that, for the participants in the
%high agreement condition, the agreement fraction for those with symmetric
%incentives is larger than that for those with high incentives on true negatives,
%but lower than for those in the remaining condition. However, given that
%participants tended to make positive predictions in the data (compared to the base
%rate), we would expect the opposite, i.e., reliance to be higher when they are
%incentivized to make negative predictions; we describe this
%pattern more in depth in Section \ref{sec:incentives_vs_predictions}. In addition, in presence of feedback the patterns that we observe
%are not entirely consistent across the three metrics.

As a confirmatory analysis,
we investigated whether any sizable effects could be detected on cases (i)
with high predictive uncertainty or (ii) where participants
were not confident about their predictions. Any effects should be most
salient on these two subsets of cases.  We performed the same regression analyses as before, but only using cases where
participants reported a level of confidence equal to 3 (out of 5) or below (and excluding participants who had more than 10 such cases, as they are likely not using the full rating scale). However, the coefficients estimates of these models were not noticeably different. In particular, we again could not find evidence that the highest level of homophily 
leads to more reliance than medium levels, nor any impact of incentives structure.
%\footnote{To further validate our results, we conducted a post-hoc analysis using a mixed-effects model. This choice is motivated by the fact that previous studies have found substantive individual differences in people’s tendency to rely on social informational sources \cite{molleman2014consistent, toelch2014individual}. Accordingly, we fitted models (logistic for binary outcomes, linear otherwise) with random effects (intercepts) for the different workers.
%to account for their propensity to rely on the AI recommendation's. 
%Effects of the interventions were captured through fixed effects. We repeated the analysis using the a binary metric of agreement between the AI and the participant, for all cases and only for the cases on which the initial predictions didn't match separately, and the influence as outcomes, measured for each defendant's case. This analysis yielded similar results to those that we report in the paper.}
% TODO: actually do this analysis

Participants were also asked about perceived
utility and trust of the AI model.
These results mirror the null findings
on the objective measures of reliance: none of the manipulations
influenced perceived utility or trust on any of the measures. More specifically, regression analyses
with perceived utility as the outcome yielded coefficients for homophily and
homophily-feedback interaction that tended in the expected directions, but were not statistically significant. 
Coefficients estimates for the high and medium homophily manipulations were of similar magnitude ($\hat\beta_H^m=0.22$ and $\hat\beta_H^h=0.25$).
%The full set of results are presented in Section \ref{sec:app_regresults}.

Prior studies have found that differential payment for types of performance can influence people's behaviors \cite{evans2004if}. No such effects were found in our experiment. In particular, participants
who received larger rewards for true negatives did \emph{not} make more negative predictions. 
We regressed proportions of
of initial (i.e., before seeing the AI recommendation) positive  predictions made by each participant for all of the manipulations, and found no statistically significant coefficient for incentives ($\hat\beta_I^n=-0.02$ and $\hat\beta_I^h=-0.02$). Additional analyses focused solely on low-confidence and high-uncertainty cases had similar results. %All results are reported in Section \ref{sec:app_regresults}. 
Moreover, there was no difference in participants' mean or median likelihood estimates as a function of incentives. 

These null results are particularly surprising since participants did seem to understand the structure of the rewards: in the final questions, 90\% of
participants reported the correct rewards for the two types of successes. Moreover, the qualitative conclusions of this analysis do not change even if we exclude the 10\% of participants who misreported the rewards structure. The lack of impact was reflected in participants' subjective experiences: of those in an asymmetric rewards condition ($N=116$), 60\% ($N=70$) reported that their predictions were either slightly or not impacted at all (mean rating for all participants of $2.2$ on a 5-point scale).


Finally, participants in the high-homophily manipulation had higher confidence  compared to the
low-agreement group ($\hat{\beta}_H^h=0.26$ with $p=0.003$, while
$\hat{\beta}_H^m=0.13$ with $p=0.12$), though their confidence decreased when they received feedback ($\hat{\beta}_{HF}^h=-0.27$ with
$p=0.007$). That is, confidence depended monotonically on homophily, unlike the other more objective measures. 
Similar results were found for perceived overall confidence between the two phases ($\hat{\beta}_H^h=0.50$ with $p<0.001$ and $\hat{\beta}_H^m=0.33$ with $p=0.004$,
but $\hat{\beta}_{AF}^h=-0.35$ with $p=0.01$). Participants overall  reported higher levels of confidence in the second phase (difference in
means=$0.17$; paired t-test $p<0.001$).
Regression analysis revealed that the observed increase was primarily due 
to the participants who experienced the lowest level of homophily, and those who received feedback in the high
homophily condition. That is, 
the high homophily condition increased participants' confidence in their
predictions only when feedback was not provided.


\subsection{Discussion}
Almost none of our initial hypotheses were confirmed by this experiment. H1 and H3 imply that participants who experience greater homophily (H1) and no feedback (H3) should have the highest levels of reliance. At the same time, participants should rely
more on the recommendations when the cost of prediction errors is asymmetric (H2). 
Although the results all trend in these directions, there is no clear impact of the sort predicted by the hypotheses. The non-monotonicity of the impact of homophily was particularly surprising, as the largest effects were found for medium levels. One possibility is that the high and low levels led participants to largely disregard the AI recommendations, though for different reasons: the former found the AI to be redundant, while the latter found the AI to be error-prone. We similarly do not find any strong effects of incentives on participants' patterns of judgments. Moreover, we find largely-null findings even though we have a reasonable sample size (roughly 27 participants per condition, each providing multiple judgments) given previously reported effect sizes for experiments such as this one.
